Full-sky Cosmic Microwave Background Foreground Cleaning Using Machine Learning

In order to extract cosmological information from observations of the millimeter and submillimeter sky, foreground components must first be removed to produce an estimate of the cosmic microwave background (CMB). We developed a machine-learning approach for doing so for full-sky temperature maps of the millimeter and submillimeter sky. We constructed a Bayesian spherical convolutional neural network architecture to produce a model that captures both spectral and morphological aspects of the foregrounds. Additionally, the model outputs a per-pixel error estimate that incorporates both statistical and model uncertainties. The model was then trained using simulations that incorporated knowledge of these foreground components that was available at the time of the launch of the Planck satellite. On simulated maps, the CMB is recovered with a mean absolute difference of $<4\mu$K over the full sky after masking map pixels with a predicted standard error of $>50\mu$K; the angular power spectrum is also accurately recovered. Once validated with the simulations, this model was applied to Planck temperature observations from its 70GHz through 857GHz channels to produce a foreground-cleaned CMB map at a Healpix map resolution of NSIDE=512. Furthermore, we demonstrate the utility of the technique for evaluating how well different simulations match observations, particularly in regard to the modeling of thermal dust.

==> diagram-source.tex <==
\begin{tikzpicture}
\sffamily
\tikzset{>=latex}
\footnotesize
\tikzset{
netnode/.style={draw, minimum size=5ex,inner sep=5pt,rounded corners},
netnodecircle/.style={draw, circle, minimum size=5ex},
learned/.style={fill=gray!20}
}

% Line break, based on https://tex.stackexchange.com/a/197922
\tikzset{ext/.pic={
\path [fill=white] (-0.2,-0.025)to[bend left](0,0.075)to[bend right](0.2,0.175)to(0.2,0.025)to[bend left](0,-0.075)to[bend right](-0.2,-0.175)--cycle;
\draw[-] (-0.2,-0.025)to[bend left](0,0.075)to[bend right](0.2,0.175) (0.2,0.025)to[bend left](0,-0.075)to[bend right](-0.2,-0.175);
}}

% ELU
\tikzset{elu/.pic={
\draw[-,thick,anchor=center,rounded corners=1mm] (-0.2,-0.1)to(0,-0.1)to(0.2,0.1);
}}

\tikzset{slash/.pic={
\draw[-] (-0.1,-0.2)to(0.1,0.2);
}}

\node[netnode] (inmap) {input map};

\node[netnode, learned, below = 5mm of inmap] (dconv1a) {$\boldsymbol\ast$};
\node[netnode, learned, right = 2mm of dconv1a] (dconv1b) {$\boldsymbol\ast$};
\node[netnodecircle, right = 2mm of dconv1b, path picture={\pic{elu};}] (dact1) {};
\node[netnode, learned, right = 2mm of dact1] (lincomb1) {$\boldsymbol\times\boldsymbol+$};
\node[left = 2mm of dconv1a] (nside1) {$\texttt{NSIDE} = \textit{N}$};
\node[below = 0mm of dconv1a] (dconvmaps1) {\emph{F}};
\node[below = 0mm of dconv1b] (dconvmaps1) {\emph{F}};

\node[netnode, below = 5mm of dact1] (pool1) {max pool};

\node[netnode, learned, below = 5mm of pool1] (dconv2a) {$\boldsymbol\ast$};
\node[netnode, learned, right = 2mm of dconv2a] (dconv2b) {$\boldsymbol\ast$};
\node[netnodecircle, right = 2mm of dconv2b, path picture={\pic{elu};}] (dact2) {};
\node[netnode, learned, right = 2mm of dact2] (lincomb2) {$\boldsymbol\times\boldsymbol+$};
\node[left = 2mm of dconv2a] (nside2) {$\texttt{NSIDE} = \textit{N}/\textit{2}$};
\node[below = 0mm of dconv2a] (dconvmaps2) {\emph{F}};
\node[below = 0mm of dconv2b] (dconvmaps2) {\emph{F}};

%\node[netnode, below = 5mm of dact2] (dbreak) {...};
\node[netnode, draw=none, below = 5mm of dact2] (dbreak) {};
\node[netnode, below = 5mm of dbreak] (pool2) {max pool};
\node[below left = -5mm and 0mm of dbreak] (nside2) {Additional downscaling};

\node[netnode, learned, below = 5mm of pool2] (dconv3a) {$\boldsymbol\ast$};
\node[netnode, learned, right = 2mm of dconv3a] (dconv3b) {$\boldsymbol\ast$};
\node[netnodecircle, right = 2mm of dconv3b, path picture={\pic{elu};}] (dact3) {};
\node[netnode, learned, right = 2mm of dact3] (lincomb3) {$\boldsymbol\times\boldsymbol+$};
\node[left = 2mm of dconv3a] (nside3) {$\texttt{NSIDE} = \textit{1}$};
\node[below = 0mm of dconv3a] (dconvmaps3) {\emph{F}};
\node[below = 0mm of dconv3b] (dconvmaps3) {\emph{F}};

\node[netnodecircle, right = 20mm of lincomb3] (usum3) {$\boldsymbol+$};
\node[netnodecircle, right = 2mm of usum3, path picture={\pic{elu};}] (uact3) {};

\node[netnode, above = 5mm of uact3] (up2) {upscale};
%\node[netnode, above = 5mm of up2] (ubreak) {...};
\node[netnode, draw=none, above = 5mm of up2] (ubreak) {};
\node[below right = -5mm and 0mm of ubreak] (nside2) {Additional upscaling};

\node[netnode, learned, above = 5mm of ubreak] (uconv2a) {$\boldsymbol\ast$};
\node[netnode, learned, right = 2mm of uconv2a] (uconv2b) {$\boldsymbol\ast$};
\node[netnodecircle, right = 2mm of uconv2b] (usum2) {$\boldsymbol+$};
\node[netnodecircle, right = 2mm of usum2, path picture={\pic{elu};}] (uact2) {};
\node[left = 0mm of uconv2a] (uconvmaps2) {\emph{F}};
\node[below = 0mm of uconv2b] (uconvmaps2) {\emph{F}};

\node[netnode, above = 5mm of uact2] (up1) {upscale};

\node[netnode, learned, above = 5mm of up1] (uconv1a) {$\boldsymbol\ast$};
\node[netnode, learned, right = 2mm of uconv1a] (uconv1b) {$\boldsymbol\ast$};
\node[netnodecircle, right = 2mm of uconv1b] (usum1) {$\boldsymbol+$};
\node[netnodecircle, right = 2mm of usum1, path picture={\pic{elu};}] (uact1) {};
\node[left = 0mm of uconv1a] (uconvmaps1) {\emph{F}};
\node[below = 0mm of uconv1b] (uconvmaps1) {\emph{F}};

\node[netnode, learned, right = 2mm of uact1] (outconv) {$\boldsymbol\ast$};
\node[below = 0mm of outconv] (outconvmaps) {\emph{2}};

\node[rectangle split, rectangle split parts=2, netnode, above = 5mm of outconv] (outmap) {output map\nodepart{two}error map};


% Connect nodes
\path[style={draw, ->}] (inmap) edge (dconv1a);
\path[style={draw, ->}] (dconv1a) edge (dconv1b);
\path[style={draw, ->}] (dconv1b) edge (dact1);
\path[style={draw, ->}] (dact1) edge (lincomb1);

\path[style={draw, ->}] (dact1) edge (pool1);
\path[style={draw, ->}] (pool1) edge (dconv2a);
\path[style={draw, ->}] (dconv2a) edge (dconv2b);
\path[style={draw, ->}] (dconv2b) edge (dact2);
\path[style={draw, ->}] (dact2) edge (lincomb2);

\path[style={draw, ->}] (dact2) --pic {ext} (pool2);
\path[style={draw, ->}] (pool2) edge (dconv3a);
\path[style={draw, ->}] (dconv3a) edge (dconv3b);
\path[style={draw, ->}] (dconv3b) edge (dact3);
\path[style={draw, ->}] (dact3) edge (lincomb3);

\path[style={draw, ->}] (usum3) edge (uact3);

\path[style={draw, ->}] (uact3) edge (up2);
\path[style={draw, ->}] (up2) --pic {ext} (uconv2a);
\path[style={draw, ->}] (uconv2a) edge (uconv2b);
\path[style={draw, ->}] (uconv2b) edge (usum2);
\path[style={draw, ->}] (usum2) edge (uact2);

\path[style={draw, ->}] (uact2) edge (up1);
\path[style={draw, ->}] (up1) edge (uconv1a);
\path[style={draw, ->}] (uconv1a) edge (uconv1b);
\path[style={draw, ->}] (uconv1b) edge (usum1);
\path[style={draw, ->}] (usum1) edge (uact1);

\path[style={draw, ->}] (uact1) edge (outconv);
\path[style={draw, ->}] (outconv) edge (outmap);

\path[style={draw, ->}] (lincomb1.north) |- ++(0,2mm) -| (usum1.north);
\path[style={draw, ->}] (lincomb2.north) |- ++(0,2mm) -| (usum2.north);
\path[style={draw, ->}] (lincomb3) -- (usum3);
\node at ($(lincomb1.north) + 0.5*(usum1.north) - 0.5*(lincomb1.north)$) [above, inner sep=4mm, align=center] {\emph{M} maps\\with \emph{F} channels};
\node at ($(lincomb2.north) + 0.5*(usum2.north) - 0.5*(lincomb2.north)$) [above, inner sep=4mm, align=center] {\emph{M} maps\\with \emph{F} channels};
\node at ($(lincomb3) + 0.5*(usum3) - 0.5*(lincomb3)$) [above, inner sep=2mm, align=center] {\emph{M} maps\\with\\\emph{F} channels};

\tikzset{cslash/.pic={
\draw[-] (-0.05,-0.1)to(0.05,0.1);
}}
\node at ([yshift=2mm]$(lincomb1.north) + 0.5*(usum1.north) - 0.5*(lincomb1.north)$) [minimum size=5ex, align=center,path picture={\pic{cslash};}] {};
\node at ([yshift=2mm]$(lincomb2.north) + 0.5*(usum2.north) - 0.5*(lincomb2.north)$) [minimum size=5ex, align=center,path picture={\pic{cslash};}] {};
\node at ($(lincomb3) + 0.5*(usum3) - 0.5*(lincomb3)$) [minimum size=5ex, align=center,path picture={\pic{cslash};}] {};


% Define style for the dashed boxes
\tikzset{dotteds/.style={draw=black,
                        dash pattern=on 2pt off 2pt,
                        rectangle, rounded corners}};

% Input channels box
\node (cbox) [draw, dotteds, fit = (inmap) (nside1) (lincomb3) (dconvmaps3)] {};
% Label input channels box
\node at (cbox.north) [above, inner sep=2mm] {Independent copies for each of \emph{M} input maps};

% Legend
\matrix (legend) [matrix of nodes, row sep=2mm, nodes={anchor=west}, below left = 6cm and 2mm of outmap.east, anchor=east]
{
  |[netnodecircle, anchor=east, path picture={\pic{elu};}]| {} & ELU \\
  |[netnodecircle, anchor=east]| {$\boldsymbol+$} & Sum inputs \\
  \node[netnode, learned, anchor=east] (lconv) {$\boldsymbol\ast$}; & \node[align=left]{Convolution\\with \emph{F} filters}; \\
  |[netnode, learned, anchor=east]| {$\boldsymbol\times\boldsymbol+$} & Scale \& bias \\
};
\node[left = 0mm of lconv] (lconvn) {\emph{F}};
% Define style for the dotted boxes
\tikzset{dotteds/.style={draw=black,
                        dash pattern=on 1pt off 1pt,
                        rectangle, rounded corners}};
\node (lbox) [dotteds, fit = (legend) (lconvn)] {};

%\node [below right = 25mm and 2mm of legend.east, anchor=east] {Note: shading denotes nodes with learned parameters};
\end{tikzpicture}

